Improving GPU Multi-Tenancy Through Dynamic Multi-Instance GPU Reconfiguration

Continuous learning (CL) has emerged as one of the most popular deep learning paradigms deployed in modern cloud GPUs. Specifically, CL has the capability to continuously update the model parameters (through model retraining) and use the updated model (if available) to serve overtime arriving inference requests. It is generally beneficial to co-locate the retraining and inference together to enable timely model updates and avoid model transfer overheads. This brings the need for GPU sharing among retraining and inferences. Meanwhile, multiple CL workloads can share the modern GPUs in the cloud, leading to multi-tenancy execution. In this paper, we observe that prior GPU-sharing techniques are not optimized for multi-tenancy CL workloads. Specifically, they do not coherently consider the accuracy of the retraining model and the inference service level objective (SLO) attainment. Moreover, they cannot accommodate the overtime dynamics (e.g., inference arrival intensity) in CL execution. In this paper, we propose MIGRator, a novel GPU reconfiguration runtime that dynamically performs GPU reconfiguration for multi-tenancy CL workloads. MIGRator is based on the recent NVIDIA multi-instance GPU (MIG) to mitigate resource contention and formulates the reconfiguration optimization into Integer Linear Programming (ILP) to dynamically identify, reconfigure, and allocate the GPU instances. MIGRator leverages the "Goodput" metric in the ILP objective function to consider both inference SLO attainment and model accuracy in the reconfiguration exploration. We evaluate MIGRator using representative multi-tenancy CL workloads. The results show our approach outperforms the state-of-the-art GPU sharing techniques (i.e., Ekya, Astraea, and PARIS) by 17\%, 21\%, and 20\%, respectively.

==> tex/7_methodology.tex <==
\section{Methodology}
\label{sec:methodology}

\noindent\textbf{DNN specifications:}
We select 6 distinct models with varying Multiply-Accumulate Operation (MACs) from Pytorch\cite{pytorch} and classify models into 3 groups (High, Medium, and Low) based on their MACs, as shown in Table \ref{tab:methodology_model_table}. 
Then we construct 8 different model combinations used in experiments, as shown in Table \ref{tab:methodology_model_combinations}.
\begin{table}[]
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \centering
    \begin{tabular}{|c|c|c|c|} \hline
        Model & GFLOPS (of batch size 1) & Group & Abbreviation\\ 
        \hline
         Bert$_{base}$ & 22.2G & High  & Bert \\ 
        \hline
         ViT$_{b\_16}$ & 17.56G & High & ViT \\ 
        \hline
         ConvNeXt$_{base}$ & 15.36G & High & ConvNeXt \\ 
        \hline
         Inception$_{v3}$ & 5.71G & Low & Inception \\ 
        \hline
         ResNet$_{50}$ & 4.09G & Low & ResNet50 \\ 
        \hline
         MobileNet$_{v2}$ & 0.32G & Low & MobilNet\\ 
        \hline
    \end{tabular}
    \caption{List of models, models' GFLOPs of batch size 1, model classifications based on MACs, and model abbreviations.}
    \label{tab:methodology_model_table}
\end{table}



\begin{table}[h]
\centering
\scriptsize
\begin{tabularx}{0.47\textwidth}{|>{\centering\arraybackslash}p{1.1cm}|>{\centering\arraybackslash}p{1.4cm}|X|}
\hline
 & Notation & Description \\
 \hline
\multirow{9}{=}{Meta variables} & $(m)$ & the inference task $(m,i)$ and retraining task $(m,r)$ of model $m$ \\
\hline

\multirow{3}{=}{Feasibility} & $F_{\lambda}^s$  & a binary variable indicating whether the configuration $\lambda$ is selected in $s^{th}$ second, if the configuration is selected, the value is set to 1; otherwise, 0. \\
\hline

\multirow{5}{=}{Guarantee completion and no interruption}& $C_{(m,r)}^s$  & a binary variable indicating the retraining task $(m,r)$ is running (value 1) or not (value 0) in the $s^{th}$ second \\
\cline{2-3}
& $RT_{(m,r)}^k$ & retraining time of the task (m,r) in seconds given a k-GPC instance \\
\cline{2-3}
\hline

\multirow{3}{=}{No \red{starvation}} & $L_{(m, i)}$ & the minimum required size of an instance that the inference task $(m,i)$ can be deployed without error \\
\hline
\multirow{6}{=}{Reconfigure GPCs} & $R_{(m,i)}^s$ & a binary variable indicating a reconfiguration is initialized (value 1) or not (value 0) for the inference task $(m,i)$ in the $s^{th}$ second \\
\cline{2-3}
& $\psi_{(m,i)}$ & the average reconfiguration overhead of task $(m,i)$ during the last retraining window in seconds\\ 
\hline

\multirow{7}{=}{Objective related variables} & $Throughput_{(m,i)}^s$ & the total throughput of task $(m,i)$ in the $s^{th}$ second \\
\cline{2-3}
& {$Completion_{m}^s$} & a binary variable indicating the completion of the retraining process of model $m$ before the $s^{th}$ second, if the retraining process is completed before $s^{th}$ second, the value is set to 1; otherwise, 0 \\
\hline
Helper variable & $\mathcal{H}$ & a large constant of value 10000 in our work \\ 
\hline
\end{tabularx}
\caption{Notations used in \ourdesign\ and corresponding descriptions. For simplicity, we use $(m,?)$ to represent either inference task $(m,i)$ or retraining task $(m,r)$.}
\label{tab:ilp_notation}
\end{table}







\begin{table}[]
    \renewcommand\arraystretch{1.2}
    \scriptsize
    \centering
    \begin{tabular}{|c|c|c|c|c|} 
    \hline
    Combination & HH-1 & HH-2 & HH-3 & HL-1 \\ 
    \hline
    \multirow{2}{*}{Models} & Bert & Bert & ViT  & Bert   \\ 
    \cline{2-5}
    & ViT & ConvNeXt & ConvNeXt & Inception  \\ 
    \hline
    % \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    % \hline
    Combination & HL-2 & HL-3 & LL-1 & LL-2 \\
    \hline
    \multirow{2}{*}{Models} & ViT & ConvNeXt & Inception & Inception \\
    \cline{2-5}
    & ResNet50 & MobileNet & ResNet50 & MobileNet \\
    \hline
    \end{tabular}
    \caption{Eight model combinations and their corresponding labels based on the model classification. For example, `HH-1' denotes a combination where both models (e.g., Bert and ViT) are classified as `High'.}
    \label{tab:methodology_model_combinations}
\end{table}

\subsection{Baselines}
\label{sec:methodology_baseline}
Spatial sharing in GPU-based systems is a crucial research area. In our experiments, we evaluate spatial sharing under three well-known paradigms: Concurrent Multiple Kernels (CMK), NVIDIA Multi-Process Service (MPS), and Multi-Instance GPU (MIG).

\noindent\textbf{CMK: }CMK is the basic of GPU space sharing that lacks explicit control over resource allocation such as SMs, memory bandwidth, and caches. In this setup, CMK provides a basic level of spatial sharing without fine-grained control.

\noindent\textbf{MPS: }For MPS, we focus on the implementation provided by Astraea\cite{spatialmps-astraea}, a representative work in this domain. Astraea dynamically assigns varying proportions of SMs to different tasks over time. It adjusts SM allocation in response to changes in inference request processing times, ensuring the satisfaction of SLO targets. 

\noindent\textbf{MIG: }In the MIG context, we examine the approach used by PARIS\cite{spatialmig-paris}, a MIG-based system. The GPC allocation is determined based on the ratio of models' MACs.
The chosen allocation in PARIS is static and remains unchanged over time. In scenarios where no existing configurations perfectly match the allocation, we select the nearest available configuration to meet the requirement. 

\subsection{Scenarios}
\label{sec:methodology_scenarios}
There are two scenarios, the pure-inference scenario, and the inference-retraining scenario, and there are two jobs in each scenario.
In both scenarios, each job has an inference task, while each job also has a retraining task in the inference-retraining scenario.
In both scenarios, we use the real-world trace from Alibaba Cluster Trace\cite{trace-alibaba} as workloads for inference tasks.
In the inference-retraining scenario, retraining tasks are launched at the beginning of each retraining window) with different amounts of resources allocated depending on the resource allocation policies of baseline works.
We use the same benchmark, NC-CIFAR10, as other continuous learning works\cite{ctn-lismartfrz,ctn-aljundi2019task,ctn-li2017learning,ctn-van2019three,ctn-xu2018reinforced} that models are trained from scratch on 2 classes of CIFAR-10\cite{cifar10}. 
Then 2 new classes are introduced at each retraining window (total 8 new classes and 4 retraining windows), and models are retrained on these classes with iCaRL\cite{incr-rebuffi2017icarl}.
Also, all inference requests are uniformly distributed into these classes.
For a fair comparison, we assume the inference accuracy of models is the same in the pure-inference scenario.
However, since both MPS-based Astraea and MIG-based PARIS only handle inference tasks, a limitation in both frameworks is the lack of a dedicated resource allocation policy for retraining tasks. To address this gap, we implement a basic policy that resources allocated to inference and retraining tasks are based on the ratio of GFLOPs.

\subsection{Metrics}
\label{sec:metrics}
For every inference request, users care not only about the timeliness (whether the inference request is returned within the SLO target) but also the correctness (whether the inference request gives a correct prediction).
Therefore, we classify an inference request as valid only if it meets both timeliness and correctness.
If either one is not met, the inference request is considered invalid.
We use an indicator function, $\mathbbm{1}(Timeliness_r\ and\ Correctness_r)$, to determine the validity value for each inference request \textit{r}.
If both timeliness and correctness are satisfied, the validity value is 1.
Otherwise, the validity value is 0.
The SLO target for each model is set as twice the inference latency of the model when utilizing the full resources of the NVIDIA A100 GPU, aligned with prior works\cite{spatialmps-servingheterogeneousATC, spatialmps-laius}.
% We define the throughput of job J in the retraining window as the sum of valid inference requests.
% We define the throughput of job J given configuration C in the retraining window as the sum of valid inference requests.

% \begin{footnotesize}
% \begin{equation}
% \label{equation:valid_throughput}
% Throughput_J = \sum\limits_{r \in \substack{inference\\ request_J}} \mathbbm{1}(Timeliness_r\ and\ Correctness_r)
% \end{equation}
% \end{footnotesize}
% Then we define the goodput of job J given configuration C as the proportion of valid inference requests to the total number of inference requests received by job J, as illustrated in Equation \ref{equation:perf_metric_model_level}.

Then we define $Goodput$ of job \textit{j} as the proportion of valid inference requests to the total number of inference requests received by job \textit{j} (Equation \ref{equation:perf_metric_model_level}), as the performance measurement for each job.
% Then we define $Goodput$ of job \textit{j} as the proportion of valid inference requests to the total number of inference requests received by job \textit{j} (Equation \ref{equation:perf_metric_model_level}), as the performance measurement for each job.

\begin{footnotesize}
\begin{equation}
\label{equation:perf_metric_model_level}
    \begin{aligned}
    % Goodput^c_j &= \frac{ \sum\limits_{r \in \substack{inference\\ request_j}} \mathbbm{1}(Timeliness^c_r\ and\ Correctness^c_r) } { iReq_j^{total} } \\
    Goodput_j &= \frac{\sum\limits_{r \in inference\ request_j} \mathbbm{1}(Timeliness_r\ and\ Correctness_r)} {inference\ request^{total}_j} 
    \end{aligned}
\end{equation}
\end{footnotesize}
% Thus, the goodput of the system under configuration C is defined as the ratio of total valid inference requests to the total number of inference requests received across all jobs (Equation \ref{equation:perf_metric_sys_level}).
% Thus, the overall goodput of the system, which is equal to the ratio of total valid inference requests to the total number of inference requests received across all jobs (Equation \ref{equation:perf_metric_sys_level}), is used to measure system performance.
Thus, we measure system performance using $Goodput_{sys}$ metric, defined as the ratio of the total number of valid inference requests to the total number of inference requests received across all jobs.
% as detailed in Equation \ref{equation:perf_metric_sys_level}. 
% This goodput metric effectively quantifies the system's efficiency in processing inference requests, serving as a comprehensive indicator of performance.

% \begin{footnotesize}
% \begin{equation}
%     \label{equation:perf_metric_sys_level}
%     \begin{aligned}
%     % Perf^C_{sys} = \frac{ \sum_{M \in Models} (Request^{total}_M \cdot Perf_M^C )}  { \sum_{M \in Models} Request^{total}_M }
%     % Goodput^c_{sys} &=  \frac{ \sum_{j \in jobs} \sum_{r \in iReq_j} \mathbbm{1}(Timeliness^c_r\ and\ Correctness^c_r)}  { \sum_{j \in jobs} iReq^{total}_j } \\
%     overall\ Goodput &=  \frac{\sum\limits_{j \in jobs}\ \sum\limits_{r \in \substack{inference\\ request_j}} \mathbbm{1}(Timeliness_r\ and\ Correctness_r)} {inference\ request^{total}_j} 
%     \end{aligned}
% \end{equation}
% \end{footnotesize}

% Similarly, we define the SLO achievement of model M given configuration C as the proportion of responses that only satisfy timeliness to the total number of received inference requests, as illustrated in Equation \ref{formula:perf_metric_model_level}.
% \begin{footnotesize}
% \begin{equation}
% \label{equation:slo_metric}
% SLO\ attainment_j = \frac{ \sum\limits_{r \in inference\ request_j} \mathbbm{1}(Timeliness_r) } { inference\ request^{total}_j}
% \end{equation}
% \end{footnotesize}




